RecXplainer: Amortized Attribute-based Personalized Explanations for Recommender Systems

Recommender systems influence many of our interactions in the digital world -- impacting how we shop for clothes, sorting what we see when browsing YouTube or TikTok, and determining which restaurants and hotels we are shown when using hospitality platforms. Modern recommender systems are large, opaque models trained on a mixture of proprietary and open-source datasets. Naturally, issues of trust arise on both the developer and user side: is the system working correctly, and why did a user receive (or not receive) a particular recommendation? Providing an explanation alongside a recommendation alleviates some of these concerns. The status quo for auxiliary recommender system feedback is either user-specific explanations (e.g., "users who bought item B also bought item A") or item-specific explanations (e.g., "we are recommending item A because you watched/bought item B"). However, users bring personalized context into their search experience, valuing an item as a function of that item's attributes and their own personal preferences. In this work, we propose RecXplainer, a novel method for generating fine-grained explanations based on a user's preferences over the attributes of recommended items. We evaluate RecXplainer on five real-world and large-scale recommendation datasets using five different kinds of recommender systems to demonstrate the efficacy of RecXplainer in capturing users' preferences over item attributes and using them to explain recommendations. We also compare RecXplainer to five baselines and show RecXplainer's exceptional performance on ten metrics.

==> CIKM2023/ablations.tex <==
\section{Ablation Experiments}

We also performed ablation experiments by removing users who rated few items. More ratings per user means that the estimation of proxy measures will be more accurate as attributes would have a higher probability of prevalence in the liked and rated item sets. Thereby, we reduce the uncertainty in the proxy measures by only considering users that rate more items than a threshold. 
% Note that Movielens datasets already filter users to have a minimum of 20 ratings per user. 
We constructed different versions of the \underline{\textsc{Movielens-$100K$}} and \underline{\textsc{Hetrec}} datasets where we filter users to have a minimum rating of different thresholds: 20, 40, 60, or 80. We then reran the experiments for these versions of the dataset and computed all the metrics. We report the trends in these metrics in \Cref{fig:ablation_increasing_min_user_rating_ml-100k} for \underline{\textsc{Movielens-$100K$}} and \Cref{fig:ablation_increasing_min_user_rating_hetrec} for \underline{\textsc{Hetrec}} dataset respectively. For \toolname, we show the metrics using the linear layer as its auxiliary model. 

\textbf{\underline{\textsc{Movielens-$100K$}}} dataset:
For all the minimum rating settings, \toolname performs the third best for the test-set and top-$k$ recommendations coverage-based metrics (behind global and user-specific popularity). For specific preference ranking, it performs the best across all settings. It performs the best for general preference coverage at lower minimum user ratings (20 and 40) and second for higher minimum user ratings (60 and 80). 

\textbf{\underline{\textsc{Hetrec}}} dataset:
For all the minimum rating settings, \toolname performs the third best for test set coverage. For recommendations coverage, it performs second best for minimum rating settings 20 and 40 and third best for minimum rating settings 60 and 80. 
For specific preference ranking and general preference coverage, \toolname consistently performs the best across all settings. 

Therefore, we can conclude that \toolname performs reliably well across a wide set of minimum user rating settings. 


==> CIKM2023/abstract.tex <==
Recommender systems influence many of our interactions in the digital world---impacting how we shop for clothes, sorting what we see when browsing YouTube or TikTok, and determining which restaurants and hotels we are shown when using hospitality platforms. Modern recommender systems are large, opaque models trained on a mixture of proprietary and open-source datasets. 
Naturally, issues of trust arise on both the developer and user side: is the system working correctly, and why did a user receive (or not receive) a particular recommendation? Providing an \emph{explanation} alongside a recommendation alleviates some of these concerns. 
The status quo for auxiliary recommender system feedback is either user-specific explanations (e.g., ``users who bought item B also bought item A'') or item-specific explanations (e.g., ``we are recommending item A because you watched/bought item B''). 
However, users bring personalized context into their search experience, valuing an item as a function of that item's attributes and their own personal preferences. 

In this work, we propose \toolname, a novel method for generating fine-grained explanations based on a user's preferences over the attributes of recommended items.
We evaluate \toolname on five real-world and large-scale recommendation datasets using five different kinds of recommender systems to demonstrate the efficacy of \toolname in capturing users' preferences over item attributes and using them to explain recommendations. We also compare \toolname to \baseline baselines and show \toolname's exceptional performance on ten metrics. 
% Our appendix is hosted at {\color{blue}{\url{https://anonymous.4open.science/r/CIKM_1244_appendix-3C48/}}}. 

% We also propose ten new evaluation metrics and compare \toolname to six baseline methods. 

%~\citep{survey-reco-xai,explicit-factors-paper-yongfeng}.
%Prior research has shown that providing recommendations along with their reason enhances trust, scrutability, and persuasiveness of the recommender systems \citep{Tintarev2007-thesis,xai-reco-motivation2,old-xai-reco-paper-sinha-2002}. 

%Recent literature in explainability has been inundated with works proposing several algorithms to this end \citep{survey-reco-xai}. 
%However, users think about items in terms of their attributes that they prefer \citep{McAuley-and-Leskovec2013,McAuley2012LearningAttributes}. 
% This motivates coupling item-specific and user-specific explanations in favor of a combined approach.
%\citep{attribute-based-xai-reco2-radarchart-paper}. 

==> CIKM2023/algorithm.tex <==
\section{\toolname: Architecture}
\label{sec:algo}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.85\columnwidth]{../plots/RecXplainer-arch.pdf}
    \caption{\toolname's architecture. It trains an auxiliary model that takes as input the learned user embeddings (from the recommender system's latent space) and an attribute vector for each item that this user rated. The item attribute vector is multi-hot -- it has 1s when the item has those attributes, else 0s. The auxiliary model aims to produce the rating originally given by the user to this item. Once trained, we use the auxiliary model to produce explanations tailored to the user's preference over item attributes.}
    \label{fig:recxplainer-architecture}
\end{figure}

\Cref{fig:recxplainer-architecture} shows the architecture of \toolname. We train a model (\emph{Auxiliary Model} in the diagram) that takes as input the concatenated vector consisting of a) a user's embedding from the trained recommender system's latent space and b) an item's attribute vector. The attribute vector is multi-hot -- it has 1s when the item has those attributes, otherwise, 0s (instead of binary values, the vector could also have continuous values). For example, consider a movie recommendation platform with metadata about the genres, and there are a total of 20 genres that movies are categorized on. A particular movie will usually belong to 1-3 genres, and hence the attribute vector of a movie would consist of 1-3 `1's in those indices (indicating the presence of those genres), and the rest of the indices will be `0's. 
The model is trained for all ratings present in the training data, and the goal is to reproduce the rating as given by the user (\texorpdfstring{\emph{R\textsubscript{orig}}}{} in the diagram). The model is trained using a mean-squared error between the original rating and the predicted rating (\texorpdfstring{\emph{R\textsubscript{pred}}}{} in the diagram). 
The auxiliary model can be instantiated with any model architecture. 
For experiments, we used three models: a linear layer, a 2-layer neural network, and a 4-layer neural network. We trained the models using Adam optimizer until convergence. 

\subsection{\toolname: Generating Explanations}
Once the auxiliary model is trained, we use it to generate explanations for recommended items. 
Given that we need to explain an item recommended to a user (a user-item pair), \toolname produces an order of that item's attributes ranked in decreasing order of the user's preference over them. We term this as the user's \emph{specific preference} over the recommended item's attributes. 
The importance of a particular attribute in a recommended item is computed as the difference in the predicted rating if that attribute was not present in the item (the auxiliary model predicts the rating). For illustration, consider a movie recommendation platform. Alice is a user of the platform and gets a recommendation for a movie whose genres are \emph{Crime}, \emph{Romance}, and \emph{Documentary}. Alice is curious why she was recommended this movie and requests an explanation: \toolname explains to Alice that she was recommended this movie because she likes \emph{Crime} movies. 

Now let us look at how \toolname arrived at this explanation: the auxiliary model predicts a rating of \textcolor{blue}{4.2} for this movie, considering Alice's watch history (captured by her embedding). (Note that the recommendation of the movie was produced by the recommender system and not the auxiliary model.)
\toolname uses the auxiliary model to predict this movie's rating if some of the genres were not present in this movie. Empirically, this is computed by zeroing out the item attribute vector at the indices of the genres whose absence we want to simulate. 

\begin{table}[h]
\centering
\caption{Illustration of how \toolname computes the specific preference of a user over an item's attributes (in this case, genres of a movie). The first row shows the rating that the auxiliary model originally predicted for the movie (\textcolor{blue}{4.2}). In the following rows, we simulate the removal of a genre at a time by zeroing out its index in the item's attribute vector and passing it through the model to compute the rating of an item that did not have that genre -- thereby capturing that genre's importance to a user. The higher the change in predicted rating when a genre is removed (rightmost column), the higher the genre's importance for a user. }
\label{tab:specific-pref}
\begin{tabular}{ccc}
        \toprule
        Genre removed & Predicted rating & $\Delta$(Predicted rating) \\ 
        \midrule
        \textcolor{gray}{All genres present}  & \textcolor{blue}{4.2} \tikzmark{a} &  --  \\
        \emph{Crime}      & 3.2 \tikzmark{b} & \tikzmark{c} 1.0  \\
        \emph{Romance}    & 3.7 \tikzmark{d} & \tikzmark{e} 0.5  \\
        \emph{Documentary} & 3.9 \tikzmark{f} & \tikzmark{g} 0.3  \\ 
        \bottomrule
    \end{tabular}
    \begin{tikzpicture}[overlay, remember picture, shorten >=.5pt, transform canvas={yshift=.25\baselineskip}]
    \draw [->] ({pic cs:a}) [bend left] to ({pic cs:b});
    \draw [->] ([yshift=6pt,xshift=2pt]{pic cs:b}) -- ({pic cs:c});
    
    \draw [->] ({pic cs:a}) [bend left] to ({pic cs:d});
    \draw [->] ([yshift=6pt,xshift=2pt]{pic cs:d}) -- ({pic cs:e});
    
    \draw [->] ({pic cs:a}) [bend left] to ({pic cs:f});
    \draw [->] ([yshift=6pt,xshift=2pt]{pic cs:f}) -- ({pic cs:g});
  \end{tikzpicture}
\end{table}

\Cref{tab:specific-pref} shows this procedure. We zero out the genres present in the movie, one at a time, and see the change in the predicted rating (the original rating is the rating produced by the auxiliary model when all the genres of the movie are considered). The higher the change, the higher the importance of the removed genre, and hence the higher it's rank (for this user). 
In the above example, Alice's \emph{specific preference} over the genres is \emph{Crime}, \emph{Romance}, and \emph{Documentary}. 
% This is \toolname's analog of \emph{local interpretability}, similar to the explanations provided by popular methods like LIME \citep{ribeiro_why_2016} and SHAP \citep{shap-paper}. 

\medskip

\toolname's approach of attributing importance to genres falls in a well-studied domain of removal-based explanation methods. There are several alternatives in the choice of removing features for attribution. We choose to remove one feature at a time. SHAP \citep{shap-paper} provides an alternative where all subsets of the features are removed to assign importance to the features using the Shapley value formula \citep{shapley:book1952}. Naturally, SHAP is much more expensive than one feature removal. \toolname is agnostic to the specific feature removal technique. \Cref{sec:removal-based} provides a comparison of using one feature removal and SHAP for feature attribution. We find that the \toolname performs slightly better when using SHAP for feature attribution, however, SHAP is much more expensive and not scalable to large datasets. 
Therefore, in the evaluation section, we use one feature removal for the main results.  
% Local interpretability methods like LIME and SHAP rank the features of an input datapoint in the decreasing order of its importance to the predicted class or value. 
% \toolname achieves this for CF-based recommender systems. 

\subsection{Global Attribute Importance}
Given the procedure to generate a user's specific preference over the attributes of a recommended item, we can capture a user's preference over all the attributes in a recommendation platform, which we term as a user's \emph{general preference}. 
\toolname computes a user's general preference by averaging the importance of each attribute over all the items that a user liked in the past. Note that since most items have a small subset of the attributes (a movie would usually belong to small set of 1-3 genres), the importance of the attributes not present in an item is set to be 0. 
% \emph{General preference} is our analog of \emph{global interpretability}  problems by LIME and SHAP. 

\emph{Specific preference} and \emph{general preference} respectively are the analogs of \emph{local interpretability} and \emph{global interpretability} provided by popular methods like LIME \citep{ribeiro_why_2016} and SHAP \citep{shap-paper}. %for classification problems. 


==> CIKM2023/best-test-loss.tex <==
\begin{table}
\caption{We train twenty-five dataset-model combination pairs. For each pair, we perform an extensive hyperparameter search to determine the lowest test loss, shown here in the table. The best performing model for each dataset is in bold. }
\label{tab:best-test-loss}
\begin{center}
\resizebox{0.9\columnwidth}{!}{%
    \begin{tabular}{cccccc}
    \hline
        Dataset/Model      & MF & AutoE     & NCF        & FM    & Deep FM    \\ \hline
        Movielens-100K & \textbf{0.82}      & 1.1            & 0.87           & 0.85                    & 0.91                        \\ \hline
        Hetrec         & \textbf{0.57}      & 0.84           & 0.62           & 0.64                   & 0.70                         \\ \hline
        Anime          & 2.1                & 1.7            & \textbf{1.5}   & 1.8                    & 2.0                        \\ \hline
        Movielens-20M  & 0.95               & 0.83           & 0.63           & 0.82                   & \textbf{0.62}               \\ \hline
        YahooMusic     & \textbf{568}     & \textit{Timeout} & 613          & 658                    & 624                       \\ \hline
    \end{tabular}%
    }
\end{center}
\end{table}



==> CIKM2023/conclusion.tex <==
\section{Conclusions}
\label{sec:conclusion}

In this work, we proposed a novel attribute-based explainability technique, \toolname, which explains recommendations for a collaborative filtering-based recommender system using the attributes of the item that a user prefers. To the best of our knowledge, \toolname is the \textbf{first and only} existing technique that provides such explanations in a post-hoc and amortized manner. We studied the performance of \toolname and \baseline baselines using five large scale recommender systems datasets trained on a variety of collaborative filtering architectures. As our results indicate, \toolname strikes an outstanding balance between coverage and personalization of the explanations and performs better than all the \baseline baselines on most metrics in all five experiments. 

The minor limitation of \toolname is the cost incurred during the training of the auxiliary model. For all five recommender systems, the training of the auxiliary model took between 10 - 30 minutes, depending on the dataset size. Once trained, these models can be used to explain recommendations for any user. The explanation generation during inference is very cheap; it took less than 10 minutes to compute the general and specific preferences for all the users, even for the largest datasets. 

We also want to mention that neither of the previous techniques, LIME-RS or AMCF, considered popularity as a baseline. We show that popularity approaches perform the best on the two coverage metrics (LIME-RS and AMCF were evaluated on these metrics). 
Through our analysis, we demonstrate the need for additional metrics to capture the personalization of the explanation, something not captured by the previously proposed coverage based metrics. 
Hence we consider proposing popularity-based approaches for explainability in recommender systems as a contribution of our work. 


% Even the item-based explainability papers \citep{Adbollahi-and-Nasraoui-constrain,Peake-and-Wang-data-mining2018} did not compare to popularity even though the metrics they considered were precision and recall. 
% Since recommender systems are known to have popularity bias \citep{Abdollahpouri2019-popularitybias1,Zhu-popularitybias2}, popular items and popular attributes can perform very well on these metrics. 



==> CIKM2023/discussion.tex <==

\subsection{Results and Discussion}

\input{table-ml-100k-matrix-fact}

\Cref{tab:5-random-seeds-ml-100k-matrix_fact} reports the ten metrics for all the baselines and \toolname for the \underline{\textsc{Movielens-$100K$}} dataset trained using \emph{Matrix Factorization} based recommender system. We now analyze the results:
\begin{enumerate}[leftmargin=*,noitemsep,topsep=-1pt]
    \item \emph{LIME-RS: }  \toolname performs better than LIME-RS on all ten metrics.  
    
    \item \emph{AMCF-PH: } \toolname performs better than AMCF-PH on nine metrics and matches in one metric. 
    
    \item \emph{Global popularity: } It achieves the highest test set and top-$k$ recommendations coverage among all techniques. Upon further analysis, we found that the three most popular movie genres \emph{Action}, \emph{Comedy}, and \emph{Drama} occur in over 88\% of the test set items (see the genre distribution plot in \Cref{fig:genre_dist_ml-100k}). Hence global popularity technique serves these three attributes as explanations for any recommendation, thus providing unpersonalized and uninformative explanations. 

    \begin{figure}[h!]
        \centering
        % \includegraphics[width=0.8\columnwidth]{../plots/genre_distribution_plots/genre_count_ml-100k.pdf}
        \includegraphics[width=0.8\columnwidth]{ml-100k_genre_distribution.pdf}
        \caption{The genre distribution for \underline{\textsc{Movielens-$100K$}} dataset. The top-3 most popular genres: \emph{Action}, \emph{Comedy}, and \emph{Drama} occur in over 88\% of the movies. And therefore, global popularity can achieve very high test set coverage while providing uninformative and unpersonalized explanations.}
        \label{fig:genre_dist_ml-100k}
    \end{figure}

    This is demonstrated by its poor performance on all personalization metrics, where it performs worse than even the \emph{random} baseline for several metrics. Therefore, we can conclude that the explanations served by global popularity technique does not capture a user's preference over attributes and performs well for the two coverage-based metrics because of the skewed distribution of the attributes. 
    
    \item \emph{User-specific popularity: } This popularity approach achieves the second highest test set and top-$k$ recommendations coverage, and similar to \emph{global popularity} performs worse than \toolname on all personalization metrics, even worse than the \emph{random} baseline on several metrics. %Since the popular genres: \emph{Action}, \emph{Comedy}, and \emph{Drama} are present in over 88\% of the movies, with a very high chance, even user-specific popularity selects them for most users. 
    
    \item \emph{Random: } We used this approach to serve as control and to ensure that no metric was trivial to perform well on. Not surprisingly, \toolname performs better than it on all ten metrics. 
    
    \item \emph{\toolname: } \toolname has the third highest test set and top-$k$ recommendations coverage while performing the best on all personalization metrics. Therefore, we can conclude that \toolname serves the most personalized explanations while still being able to explain a large proportion of test set items and top-$k$ recommendations. Moreover, \toolname can provide explanations in an amortized manner, saving a lot of compute during inference time. 
\end{enumerate}

\input{table-hetrec-matric-fact}

\Cref{tab:5-random-seeds-hetrec-matrix_fact} reports the ten metrics for all the baselines and \toolname for the \underline{\textsc{Hetrec}} dataset trained using \emph{Matrix Factorization} based recommender system. We analyze the results:
\begin{enumerate}[leftmargin=8pt,noitemsep,topsep=-1pt]
    \item \emph{LIME-RS: }  \toolname performs better than LIME-RS for eight out of ten metrics and matches in one metric. 
    
    \item \emph{AMCF-PH: } \toolname performs better than AMCF-PH on all ten metrics. 
    
    \item \emph{Global popularity: } Similar to Movielens-$100K$, global popularity performs the best for the test set and top-$k$ recommendations coverage. This is due to the skewed distribution of genres (see \Cref{sec:attribute-dist-plots}). It performs worse than \toolname (even worse than the \emph{random} baseline) for all personalization metrics. 
    
    \item \emph{User-specific popularity: } Similar to Movielens-$100K$, user-specific popularity performs the second best for the test set and top-$k$ recommendations coverage, and worse than \toolname (even worse than \emph{random} baseline) for all personalization metrics. 
    
    \item \emph{Random: } As expected, \toolname performs better than the random baseline performs on all ten metrics. 
    
    \item \emph{\toolname: } \toolname performs the third best for test set coverage and the second best for top-$k$ recommendations coverage. It also performs the best for seven out of eight personalization metrics. This demonstrates that \toolname provides personalized explanations to the user while providing high coverage.
\end{enumerate}

\input{table-ml-20m-dfm}

\Cref{tab:5-random-seeds-ml-20m-dfm} reports the ten metrics for all the baselines and \toolname for the \underline{\textsc{Movielens-$20M$}} dataset trained using \emph{Deep Factorization Machine} based recommender system. We analyze the results:
\begin{enumerate}[leftmargin=*,noitemsep,topsep=-1pt]
    \item \emph{LIME-RS: } Recall that LIME-RS trains a separate regression model for each item to be explained to each user. This is a very expensive procedure to generate explanations. For a large dataset like Movielens-20M that has 138,000 users, LIME-RS did not scale. LIME-RS took more than 1 hour to compute the general preferences for just 1000 randomly sampled users -- thereby, its estimated computation time for both the specific and general preferences is \textit{over 11 days}. %We, therefore, did not compute LIME-RS explanations. 
    
    \item \emph{AMCF-PH: } \toolname performs better than AMCF-PH on all ten metrics.  
    
    \item \emph{Global popularity: } Similar to the two previous datasets, global popularity performs the best for the test set and recommendations coverage, while performing worse than \toolname and even the \emph{random} baseline on all personalization metrics. 
    
    \item \emph{User-specific popularity: } Similar to the two previous datasets, user-specific popularity performs the second best for the test set and recommendations coverage, while performing worse than \toolname and even the \emph{random} baseline on all personalization metrics. 
    
    \item \emph{Random: } As expected, \toolname performs better than the random baseline performs on all ten metrics. 
    
    \item \emph{\toolname: } \toolname performs the third best on the two coverage metrics and performs the best on all eight personalization metrics, thereby demonstrating its ability to provide personalized explanations with high coverage. 
\end{enumerate}

\input{table-anime-ncf}

\input{table-yahoo-matrix-fact}

\Cref{tab:5-random-seeds-anime-ncf} and \Cref{tab:5-random-seeds-yahoomusic-matrix_fact} reports the metrics for the \underline{\textsc{Anime}} and \underline{\textsc{YahooMusic}} datasets respectively. We analyze the results below:
\begin{enumerate}[leftmargin=*,noitemsep,topsep=-1pt]
    \item \emph{LIME-RS: } LIME-RS cannot scale to both these datasets (overall, it did not scale for 3 out of 5 datasets). For the Anime dataset, the estimated computation time for specific and general preferences is over 3 days; for the YahooMusic dataset, the estimated computation time is over 18 days. 
    
    \item \emph{AMCF-PH: } \toolname performs better than AMCF-PH for all ten metrics and nine out of ten metrics for Anime and YahooMusic datasets respectively. %Nevertheless, AMCF-PH performs better than \toolname for a couple of personalization metrics -- however, \toolname is within a percentage point for all these cases. 
    
    \item \emph{Global popularity: } For Anime dataset, global popularity performs the best on converage metrics, however, \toolname performs better than it for YahooMusic dataset on those metrics. 
    \toolname performs better than global popularity on seven out of eight and all eight personalization metrics for Anime and YahooMusic datasets respectively. 
    
    
    \item \emph{User-specific popularity: } User-specific popularity performs the second best for the Anime dataset and the best for YahooMusic dataset on the coverage metrics. \toolname performs better than user-specific popularity on five out of eight and six out of eight personalization metrics for Anime and YahooMusic datasets respectively. 
    
    \item \emph{Random: } As expected, \toolname performs better than the random baseline performs on all ten metrics for both datasets. 
    
    \item \emph{\toolname: } For coverage metrics, \toolname performs the third best for the Anime dataset and the second best for the YahooMusic dataset. It performs the best on five out of eight personalization metrics for both the datasets. (it is less than a two percentage points away from the best performing techniques for the remaining three personalization metrics for YahooMusic dataset). 
\end{enumerate}

From the experimental results, we can conclude that 
\toolname performs better than all baselines for most metrics. When it does perform worse, it is usually within a couple percentage points of the best performing technique. 
LIME-RS usually does not perform well on any metric and is unable to even scale to 3 out of 5 datasets. 
AMCF-PH also does not perform will on most metrics in all experiments. 
Global and user-specific popularity perform very well on the coverage-based metric; however, that is due to the skewed distribution of the attributes, and their explanations are usually uninformative and generic. 

In \Cref{sec:ml-100k-all-archs}, we repeat experiments for all the five architectures for \underline{\textsc{Movielens-100K}} dataset. The goal is to demonstrate the effectiveness of \toolname to provide explanations across a wide variety of collaborative filtering models. From the results, we can conclude that \toolname indeed performs well on all metrics across the five architectures, demonstrating its generalizability. 
% The conclusions from the results are similar to the aforementioned ones. 

In \Cref{sec:case-studies}, we dive into two case studies demonstrating the explanations \toolname provides for two real users from the \underline{\textsc{Movielens-100K}} dataset. 

% Due to space limitations, our full appendix is hosted at {\color{blue}{\url{https://anonymous.4open.science/r/CIKM_1244_appendix-3C48/}}}. 


==> CIKM2023/evaluation.tex <==
\section{Evaluation}
\label{sec:eval}

Our experiments characterize the quality of explanations for every user by the number of liked items in the user history and the number of top-$k$ recommendations that can be explained. 

\subsection{Datasets and Recommender Systems}
To demonstrate the scalability of \toolname, we experiment with several popular recommender datasets of increasing size. 
We trained each dataset using five popular recommender system model, and choose the model that achieved the lowest loss for each dataset. 

\input{best-test-loss.tex}

We train several models of the same architecture for each dataset with different hyperparameters, and \Cref{tab:best-test-loss} shows the model that achieved the lowest loss for each dataset. 
From the five models, the model with the lowest test loss for a dataset is chosen (highlighted in bold in the table) as the recommender system that \toolname explains. 

% To demonstrate the generalizability of \toolname, we trained five classes of recommender system architectures using these datasets:
\begin{enumerate}[leftmargin=*,noitemsep,topsep=-1pt]
    \item \underline{\textsc{Movielens-$100K$}} \citep{movielens-dataset} dataset is trained using \emph{Matrix Factorization} model. This dataset has 100,000 ratings for 1,700 movies provided by 1,000 users. Each rating is an integer from 1 to 5, with a higher rating meaning a higher likeness for the movie. The dataset also contains the genre of each movie, and there are a total of 18 genres in the dataset: \emph{Action, Adventure, Animation, Children's, Comedy, Crime, Documentary, Drama, Fantasy, Film-Noir, Horror, Musical, Mystery, Romance, Sci-Fi, Thriller, War, Western}. Each movie usually belongs to 1-3 genres. 

    \item \underline{\textsc{Hetrec}} \citep{grouplensHetRec2011} dataset is trained using \emph{Matrix Factorization} model. This dataset has 855,000 ratings for 10,100 movies provided by 2,100 users. Similar to \emph{Movielens-$100K$}, this dataset has integer ratings from 1 to 5, and each movie has genre annotations. There are 20 genres in the dataset; it shares the 18 with \emph{Movielens-$100K$} and has two additional genres: \emph{IMAX} and \emph{Short}. 

    \item \underline{\textsc{Anime}} \citep{kaggleAnimeRecommendations} dataset is trained using \emph{Neural Collaborative Filtering} model. This dataset has 6.1 million ratings for 6,500 animes provided by 47,000 users. Each rating is an integer from 1 to 10. Each anime belongs to 1-4 genres from a total set of 49 genres. 

    \item \underline{\textsc{Movielens-$20M$}} \citep{grouplensMovieLens20m} dataset is trained using \emph{Deep Factorization Machine}. This dataset has 20 million ratings for 27,000 movies provided by 138,000 users. Similar to \emph{Movielens-$100K$}, this dataset has integer ratings from 1-5, and each movie has genre annotations. There are 19 total genres in the dataset; it shares the 18 with \emph{Movielens-$100K$} and has one additional genre: \emph{IMAX}.

    \item \underline{\textsc{YahooMusic}} \citep{yahoomusicdataset} dataset is trained using \emph{Matrix Factorization} model. This dataset has 32.6 million ratings for 128,000 tracks or albums provided by 75,000 users. Each rating is an integer between 0 and 10. Each track or album has 1-5 genre annotations from a total set of 41 genres. 

\end{enumerate}

\noindent For all the datasets, we used 70\% of the data for training and validating the recommender models and 30\% of the data as the test set for computing the metrics in the next section. 

\subsection{Metrics}
We measure an approach's performance using ten metrics. The metrics can be categorized into two broad categories: \textit{coverage} of recommended items and \textit{personalization} to the user. Previous work has mostly used coverage based metrics. We argue about the insufficiency of coverage based metrics and propose a set of eight metrics that measure the personalization of the explanations to the users. These metrics can be used to evaluate any attribute-based explanation method for recommender systems. %We evaluate both general and specific preferences in these metrics. 
\begin{enumerate}[leftmargin=*,noitemsep,topsep=-1pt]
    \item \emph{Test set coverage: } This metric finds the percentage of the test set items whose attributes intersect with the top-$k$ general preferences of a user. For example, suppose a technique identifies the top-3 general preferences of a user Adam as \emph{Action}, \emph{Comedy}, and \emph{Sci-Fi}. If Adam likes a movie whose genres are \emph{Action} and \emph{Romance}, it is counted as covered by a technique as \emph{Action} had been identified as one of Adam's preferred genres. Conversely, had the movie belonged to \emph{Crime} and \emph{Adventure} genres, it would not have been covered. We measure this metric only for the items that a user liked. We consider an item `liked' if a user has rated it $4$ or higher (when the dataset ratings are between 1 and 5) and $7$ or higher (when the dataset ratings are between 1 and 10). We only consider the top-$k$ general preferences for a user when measuring coverage, where k is about 0.2 times the number of attributes in the dataset. We report the mean coverage over all the users for this metric. 
    
    \item \emph{Top-$20$ recommendations coverage: } Similar to test set coverage, this metric finds the percentage of the top-$20$ recommended items whose attributes intersect with the top-$k$ general preferences of a user. We report the mean coverage over all the users for this metric. 
\end{enumerate}

    \textbf{Insufficiency of coverage based metrics:} Since a few attributes in most recommender datasets are very popular, i.e., they occur in almost all items: identifying such an attribute as a user's preference will provide a very high test set and recommendations coverage. However, those attributes can be inaccurate, non-personalized, or uninformative as an explanation. For example, consider a movie recommendation dataset containing language as one of the attributes, where most movies are English movies. If an explanation technique provides `English' as an explanation for the recommended movie; that technique will get a 100\% test set and recommendations coverage while being uninformative and unpersonalized to the users. 
    Therefore, we propose a new set of metrics to measure the personalization of the explanations. 

\begin{enumerate}[resume,leftmargin=2pt,noitemsep,topsep=-1pt]
    \item \emph{Personalization of the explanations: } 
    To measure the personalization of the explanations we require the ground-truth information about the users' preferences over the set of attributes. However, this information is usually missing from the recommendation datasets. 
    To overcome this limitation, we propose two measures that act as reasonable proxies for a user's attribute preference: (The gold standard would be to conduct a user study; however, that would involve collecting a new recommender dataset and asking users to tell us about their preferences. We leave this to future work.)
    
    \begin{enumerate}[leftmargin=*,noitemsep,topsep=-1pt]
        \item \emph{Conditional Probability of Liking given an attribute is present: } This computes the probability that a user likes an item, given that an attribute is present in it. This measure is the ratio of the number of times an attribute is present in the items a user likes (e.g., rated 4 or higher) and the number of times it is present in all the items the user rated (e.g., rated 1 to 5). 
        
        \item \emph{Odds of Liking vs. Disliking given an attribute is present: } This computes the ratio of the number of times an attribute is present in an item the user likes (e.g., rated 4 or 5) and the number of times it is present in an item that the user dislikes (e.g., rated 1 or 2). 
        
    \end{enumerate}

    We use the training set for computing both these proxy measures. 
    Both measures provide a reasonable proxy of users' general preference over attributes, i.e., a ranked order of the attributes. Now, considering the two proxies as a ground truth of user preference over attributes, we report four personalization metrics for each of them: 
    \begin{enumerate}[leftmargin=*,noitemsep,topsep=-1pt]
        \item \emph{General preferences coverage:} This metric computes if there is any intersection between the top-$k$ attributes in a user's general preferences identified by a technique and the top-$k$ preferences identified by a proxy measure. We report the mean coverage over all the users for this metric. 
        
        \item \emph{General preferences ranking:} This metric measures the similarity between the ranking of the top-$k$ attributes in a user's general preferences identified by a technique and the top-$k$ general preferences identified by a proxy measure. 
        We use rank-biased overlap (RBO) as a measure of similarity between the two ranked lists. RBO has several advantages over traditional rank similarity metrics like Kendall's Tau or Spearman's correlation and we provide further details in \Cref{sec:rbo-just}. %, specifically that the two attribute lists need not be conjoint and RBO can provide a weighted comparison (more details in \Cref{sec:rbo-just}). 
        For a user, we compute this metric for all the items they liked in the ratings and report the mean score over all the users. 
        
        \item \emph{Specific preferences coverage:} Similar to general preferences, we also measure if there is any intersection between the top-$k$ attributes of an item as ranked by specific preferences by a technique and the top-$k$ specific preferences identified by a proxy measure. For a user, we compute this metric for all the items they liked in the ratings and report the mean coverage over all the users. 
        % for each item that a user liked in the training set (specific genre preference for a user-item pair) and the top-$k$ genre preferences identified for this user by either of the two proxies. 
        
        \item \emph{Specific preferences ranking:} We also measure the similarity in the ranking of the top-$k$ attribute of an item as ranked by specific preferences by a technique and the top-$k$ specific preferences identified by a proxy measure. We use RBO for computing the similarity between ranked attributes. For a user, we compute this metric for all the items they liked in the ratings and report the mean score over all the users. 
        
    \end{enumerate}
    Hence we have a total of eight metrics for measuring the personalization of the explanations. 
\end{enumerate}


\subsection{Baselines}
We compare \toolname to \baseline baseline approaches:
\begin{itemize}[leftmargin=*,noitemsep,topsep=-1pt] %,itemsep=2pt]
    \item \emph{LIME-RS~\citep{limers-paper}: } This is the only previous post-hoc attribute-based explainability approach for CF-based recommender systems. It trains a regression model for every item it needs to explain; hence, this approach is not amortized. As we will see later in the experimental results, LIME-RS does not scale to large datasets owing to this problem. 
    
    \item \emph{AMCF~\citep{amcf-paper}: } This is another attribute-based explainability method for CF-based recommender systems; however this technique is not a post-hoc method. It trains a model while the recommender system is being trained and requires modification in its architecture. For a fair comparison, we adapted AMCF to be post-hoc: \emph{AMCF-PH} (details in \Cref{sec:amcf-post-hoc-adapt}). We froze the recommender system and trained AMCF's model till convergence. Note that unlike our approach, AMCF takes as input the item embedding and hence does not apply to recommender systems that do not construct item embeddings explicitly, for example, autoencoder and RBM-based recommender systems. 
    % \item \emph{AMCF-PH: } The AMCF approach adapted for being post-hoc (details in \Cref{sec:appendix}). 
    
    \item \emph{Global popularity: } This approach finds the most popular attributes across the entire dataset, i.e., the attributes that are the most popular among all the items that are liked across the entire dataset. For every recommended item, this technique would serve the same explanation. It is immediately evident that the explanations will not be personalized to the users and might be uninformative depending on the attributes (recall the `English' attribute in movies example).   %For \textsc{Movielens-$100K$}, these were \emph{Action}, \emph{Comedy}, and \emph{Drama}. 
    
    \item \emph{User-specific popularity: } This approach finds the most popular attributes across the items that a particular user liked in the dataset. These explanations are more personalized to the user than global popularity; however, they can still be uninformative if a feature exists in all liked items. 
    
    \item \emph{Random: } This baseline is for control. It selects a random set of attributes for each item to be explained when computing both specific and general preferences. 
\end{itemize}

For \toolname, we use three auxiliary models in the experiments: a simple linear layer, a two-hidden layer neural network, and gradient boosted trees. In the results table, they are respectively denoted using RX-Linear, RX-MLP, and RX-GBDT. 
We repeated all experiments for five random splits of the dataset and report the mean and the standard deviation over the metrics.


==> CIKM2023/intro.tex <==
\section{Introduction}
\label{sec:intro}
Recommender systems direct our attention, telling us what to look at---and what not to. They are deployed widely at platform companies such as Netflix, YouTube, Yelp, Amazon, and Shein. There are two main approaches to generating recommendations~\citep{Adomavicius2005Toward,recobroad1}: content-based~\citep{content1,content2} and collaborative filtering~\citep{collab-reco,colab1}. Content-based systems use item attributes and/or user preferences to recommend new items, while collaborative filtering (CF)\ uses the wisdom of the crowd, based on user ratings. Hybrid recommender systems aim to combine both approaches~\citep[see, e.g.,][]{Burke2004HybridRS}.
%
Modern methods are opaque in their performance and their servicing of an end-user's needs~\citep[see, e.g.,][]{survey-reco-xai}, which we focus on in this paper. 

%Recommender systems drive the modern discovery of subjects of interest. Examples are ubiquitous, Netflix and YouTube for entertainment, Yelp for restaurants, Amazon and Shein for fashion. 
%Content-based and collaborative filtering (CF) are the two primary approaches of generating recommendations \citep{Adomavicius2005Toward,recobroad1}. Content-based recommender systems use the similarity between an item’s attributes and a user’s preference over them to recommend new items, for example recommending \textit{Top Gun} to a user who likes \emph{Action} movies \citep{content1,content2}. Collaborative filtering (CF) methods instead rely on the wisdom of the crowd to generate recommendations. Such methods are trained only using the ratings provided by the users of a recommendation platform like Netflix. The idea is that if two users have a similar rating pattern, then the items liked by a user can be recommended to the other (if they have not already interacted with it) \citep{collab-reco,colab1}. Hybrid recommender systems aim at combining the two approaches \citep{Burke2004HybridRS}. 

\begin{figure}[h]
    \centering
    \includegraphics[width=0.7\columnwidth]{../plots/recxplainer-fig1.pdf}
    \caption{A user of a fashion website is recommended a garment, about which she is wondering why that particular garment was recommended? \toolname explain that it was recommended because the user has shown interest in \textit{green} clothes and clothes from \textit{H\&M}. }
    \label{fig:recxplainer-in-action}
\end{figure}

In recent years, CF-based methods have been widely chosen over content-based methods owing to 1) no requirement of manual labeling of item features, and 2) more serendipitous recommendations \citep{google-cf-serendipitious}. (Content-based recommender systems require each new item to be featurized, whose cost is usually high \citep{pandora-content-based}.)
However, CF-based methods have one major limitation: lack of interpretability. 
CF methods map users and items to an embedding space, which is learned from the user-item interaction matrix---and the proximity in this space is used to generate recommendations. Such an embedding space is difficult to interpret. A core challenge is understanding what a model learns about the user's preference over the items' attributes and explaining how it generates the recommendations. 
% On the other hand, content-based methods are transparent and scrutable as they generate recommendations by utilizing a user's attribute preference. 
\smallskip

Previous research has established that providing explanations for a recommendation enhances the transparency, scrutability, trustworthiness, effectiveness, persuasiveness, efficiency, and satisfaction of the recommender systems \citep{Tintarev2007-thesis,xai-reco-motivation2,old-xai-reco-paper-sinha-2002}. This has spurred significant research in the broad field of ``explainability for CF recommender systems.'' 
Providing explanations when using CF-based methods is nontrivial due to the lack of interpretability of the embedding space. 
Most of the previous approaches provide explanations in the form of user-based or item-based explanations. User-based explanations explain a recommendation on the basis of `similar' users liking it. And item-based explanations explain a recommendation on the basis of its similarity to other items that the user has liked in the past. 
Item-based explanations are usually easier to grasp as the user knows about the items they have interacted with in the past. 
However, both of these explanation formats do not capture a user's preference over the attributes of an item — which is how users inherently think about a recommendation \citep{attribute-based-xai-reco2-radarchart-paper,attribute-based-xai-reco3-tagplanations-paper,attribute-based-xai-reco1,McAuley-and-Leskovec2013,McAuley2012LearningAttributes,rl-approach-xai-reco-MSFT}. 

This work proposes a novel approach, \toolname, that generates attribute-based explanations for CF-based recommender systems. 
A recommendation is explained in terms of a user's preference over the attributes of the item, (see \Cref{fig:recxplainer-in-action}), e.g., `We are recommending this movie because you like \emph{Action} movies.' or `We are recommending this t-shirt because you like \emph{Adidas} products and \emph{blue} clothes.' 
Such explanations are personalized to the user and hence help further enhance the persuasiveness and trustworthiness of the recommender systems. Note that the CF-based recommender system usually does not use these attributes to generate recommendations. 

\toolname learns a model of the user's preference over the attributes of the items and uses this model to explain novel recommendations. The key advantages of \toolname are that it a) provides post-hoc explanations, b) is model-agnostic, and c) generates explanations in an amortized fashion. 
Post-hoc explanation techniques provide explanations after the recommender systems have been trained and therefore do not interfere with their architecture or training routine. 
This is crucial for real-world recommender systems whose architectures are complex, and whose training routines are highly optimized for accuracy. Moreover, such explainability techniques evade the accuracy-interpretability trade-off \citep{rl-approach-xai-reco-MSFT,Peake-and-Wang-data-mining2018}. 
Model-agnostic explanation techniques are desirable for their flexibility and generalizability as they can be used to explain a broad class of recommender systems \citep{molnar2022-xaibook}. 
% Previous research has also established the significance of post-hoc and model-agnostic explainability, citing two primary reasons: 1) no accuracy-interpretability trade-off (simpler and interpretable models are usually less accurate); and 2) generalizability to a wide class of recommender systems . 
Moreover, \toolname generates explanations in an amortized fashion, i.e., once \toolname learns the user's preference over attributes, it can generate explanations for novel recommendations by merely doing a model inference -- that is very cheap and hence scalable to large scale recommender systems. 

We found that the important intersection of post-hoc attribute-based explanations for CF-based recommender systems has not garnered sufficient attention in explainability literature. 
We are aware of only two previous approaches that generate attribute-based explanations for CF-based recommender systems: LIME-RS \citep{limers-paper} and AMCF \citep{amcf-paper} (details in \Cref{sec:related}). 
LIME-RS did not evaluate its attribute-based explanations, and the metrics used by AMCF were not generalizable to all CF-based recommender systems (see \Cref{sec:amcf-metrics-bad}). To this end, we propose a set of eight generalizable metrics to evaluate attribute-based explainability techniques for recommender systems (\Cref{sec:eval}) (one of our major contributions). We also consider the often overlooked popularity-based explanation methods: for attribute-based explanations, such an approach would choose the most popular attributes of a recommended item as an explanation. In this work, we implemented three popularity-based baselines for a holistic evaluation. 
%Overall, we do an extensive benchmarking of LIME-RS, AMCF, popularity based baselines, and \toolname along over several large scale recommender systems and datasets in this work. 

In summary, our contributions are as follows:
\begin{enumerate}[leftmargin=*,topsep=0pt,itemsep=2pt]
    \item We propose \toolname, a novel, post-hoc, and model-agnostic technique to provide attribute-based explanations for recommender systems in an amortized fashion. To the best of our knowledge, \toolname \textbf{is the first technique} to have all these desirable properties. 
    
    \item We propose novel metrics to evaluate attribute-based explainability methods for CF-based recommender systems. % that can be used to compare all future techniques. 
    
    \item We perform extensive experimentation with five different classes of recommender systems trained on five large scale recommendation datasets. We demonstrate the efficacy of \toolname and its comparison with \baseline baselines using ten metrics. We observe that \textit{\toolname outperforms all the baselines for about eight out of the ten metrics across all experiments}. 
    
    \item We also explore the comparison of \toolname with the often overlooked popularity-based explanation methods, revealing surprising results. 
\end{enumerate}





==> CIKM2023/related.tex <==
\section{Related Work}
\label{sec:related}
In this section we provide a brief review of relevant works that cover the general topic of explainability in recommender systems, as well as post-hoc explainability and attribute-based explainability as specific topics. 

\subsection{Explainability in Recommender Systems}
Explainable recommender systems provide recommendations along with an explanation for doing so. The term `explainable recommendation' was introduced by \citet{explicit-factors-paper-yongfeng} in \citeyear{explicit-factors-paper-yongfeng}; however, papers were talking about the benefits of providing explanations much earlier \citep{Tintarev-cfe-xai-survey-2007,Tintarev2011,old-xai-reco-paper-sinha-2002}. 

Most previous methods for explainability in collaborative filtering-based (CF-based) recommender systems provide explanations in user-based or item-based fashion \citep{survey-reco-xai}. 
The approaches that generate these explanations can either be model-specific or model agnostic, the former kind constituting the majority of previous approaches. 
Models-specific approaches train inherently interpretable models by either constraining the embedding space or developing custom recommender system architectures that are not usually generalizable. For example, \citet{explicit-factors-paper-yongfeng} propose extracting user preferences over attributes from their reviews and using that to provide explanations for recommendations. The authors train an explicit factor recommender model that takes the user's preference over attributes as input during training the recommender model. Such an approach is restricted to situations where the user reviews over items are available in abundance and also might suffer from the accuracy-interpretability trade-off. 
In another approach, \citet{Adbollahi-and-Nasraoui-constrain} add constraints to the latent space of the matrix factorization models to encourage explainability. Even though their approach only provides user and item-based explanations, it lands deep in the accuracy-interpretability trade-off debate. 
There exist many other approaches in this category \citep{Chen2016,Chen2018,Bauman2017,Tao2019,Liu2019,McAuley-and-Leskovec2013,EX3-yongfeng-paper}. 
As evident, the major downside of these approaches is that they are \emph{not} post-hoc, i.e., they need to modify the recommender system architecture in order to provide explanations -- and this is problematic for two reasons: 1) there is a potential accuracy-interpretability trade-off, and 2) real-world recommender systems are trained and fine-tuned over large datasets, and their developers are rarely willing to train a new model from scratch in order to provide explanations \citep{varshney}. 
Hence post-hoc explainability techniques attract a lot of attention, especially from an industry perspective \citep{verma2021amortized,molnar2022-xaibook}. 

\subsection{Post-hoc Explainability in Recommender Systems}
There only exist a handful of explainability techniques in this category. 
\citet{Peake-and-Wang-data-mining2018} use a data-mining approach to provide item-based explanations in a post-hoc manner. 
\citet{limers-paper} propose LIME-RS which draws motivation from the original LIME paper \citep{ribeiro_why_2016}. LIME-RS samples items close to a recommended item, and learns a linear regression model on these samples, and uses the regressor to provide an explanation that can be either item-based or attribute-based (the latter can be provided if the attributes of the items are appended to the items embeddings when training the regression model). LIME-RS is the only previous approach that provides attribute-based explanations for CF-based recommender systems and is a post-hoc explanation technique. However, LIME-RS is not amortized -- it trains a separate regression model for each recommended item and hence is not scalable to large scale datasets (see \Cref{sec:eval} for evaluation of LIME-RS on large scale datasets). 
\citet{FIA-paper-Cheng2019} propose a technique that uses influence functions to find the influence of training ratings on a particular recommendation, and the ratings with the greatest influence are served as explanations. Hence, this technique also only provides item-based explanations. 

\subsection{Attribute-Based Explainability in Recommender Systems}
Unlike user-based and item-based explanations, attribute-based explanations explain a recommendation based on the user's personalized attribute preferences, thereby enhancing the system's overall persuasiveness and trustworthiness \citep{attribute-based-cfe-reco-RL,attribute-based-xai-reco1}. 
As mentioned earlier, there do exist previous works that provide explanations that utilize the user's preference over interpretable attributes of an item. Most of these works utilize the reviews provided by the users to capture this preference (and use that to train the recommender system itself \citep{explicit-factors-paper-yongfeng,McAuley-and-Leskovec2013,attribute-based-xai-reco2-radarchart-paper}). However, such reviews might not exist even in the presence of ratings. For example, Netflix scrapped its review section due to low user participation recently \citep{netflix-no-more-reviews}. 
Secondly, there is no guarantee of mention of interpretable attributes in the reviews that can be used to learn the user's preference. Even the datasets used in these approaches had very sparse user reviews; over 77\% of the users had only \emph{one review} \citep{attribute-based-xai-reco4-trirank-paper}, making the inference of users' preferences challenging. 

On the other hand, \toolname also provides attribute-based explanations; however, it utilizes the attributes of an item that is available in their metadata, e.g., movie or game genres, and hence \emph{does not} depend on user reviews. 
Similar to ours, AMCF \citep{amcf-paper} learns users' preferences over item attributes by training an attention network. So it provides attribute-based explanations like our approach; however, AMCF is not a post-hoc technique -- it needs to be trained along with the recommender system. 
Similarly, \citet{attribute-based-cfe-reco-RL} proposes CERec to determine the attributes that are important for a user-item pair (in a counterfactual manner); however, CERec is also not a post-hoc technique. 
\citet{rl-approach-xai-reco-MSFT} propose a post-hoc RL-based approach that generates attribute-based explanations for a user; however, like most previous approaches, it acquires the attributes from the user reviews -- whose downsides are aforementioned. 
Hence our approach sits at the intersection of attribute-based (\emph{without} requiring user reviews), post-hoc explanation techniques, generating amortized explanations. 
To the best of our knowledge, \toolname \textbf{is the first technique} to have all these desirable properties. 
% (note that LIME-RS is still not amortized and does not scale to large datasets). 


% \subsection{Evaluation Metrics for Explainability of Recommender Systems}
% \todo{When doing the full version of the paper, we can write a subsection on metrics of explainability for recsys -- talk about https://xaitutorial2020.github.io/raw/master/slides/aaai_2020_xai_tutorial.pdf and https://arxiv.org/pdf/2106.07758.pdf} 


==> old-ml-100k-results.tex <==
\begin{table}[h]
	\caption{The test set coverage, top-k recommendations coverage, and the 8 explanation personalization metrics are reported here (averaged over all users) for the \textbf{MovieLens-100K} dataset. For \toolname, we computed metrics with three auxiliary models: Linear, a 2-layer neural network (MLP1), and a 4-layer neural network (MLP2). For all columns, a higher value is better. The highest value for each metric is emboldened. }
	\begin{center}
	\resizebox{1.0\columnwidth}{!}{%
		\begin{tabular}{llllllllll}
			\toprule
			Metrics & LIME-RS & AMCF & AMCF-PH & GBL Popl. & User Popl. & Random & Our-Linear & Our-MLP1 & Our-MLP2 \\
			\midrule
			Testset Coverage & 8.4 & 47.2 & 52.6 & \textbf{84.5} & 77.9 & 32.4 & 60.7 & 70.8 & 71.2 \\
			Recommendations Coverage & 26.0 & 44.3 & 46.1 & \textbf{73.2} & 69.6 & 30.6 & 61.3 & 68.6 & 67.8 \\
			CondProb Generalpref Coverage & 50.3 & 58.2 & 47.2 & 29.0 & 41.8 & 43.9 & \textbf{62.9} & 58.1 & 56.6 \\
			CondProb Generalpref Ranking & \textbf{15.8} & 15.1 & 11.2 & 5.8 & 9.9 & 11.0 & 15.2 & 14.0 & 13.8 \\
			CondProb Specificpref Coverage & 52.5 & 53.1 & 52.4 & 29.0 & 41.7 & 44.1 & \textbf{55.3} & 53.8 & 53.6 \\
			CondProb Specificpref Ranking & 14.6 & 49.6 & 50.3 & 6.8 & 10.4 & 11.0 & \textbf{52.2} & 50.7 & 51.2 \\
			Odds Generalpref Coverage & 32.6 & 63.7 & 60.4 & 48.5 & 55.0 & 43.7 & \textbf{73.4} & 72.3 & 70.4 \\
			Odds Generalpref Ranking & 9.4 & 19.4 & 18.0 & 18.2 & 26.7 & 10.6 & 25.6 & 27.6 & \textbf{28.2} \\
			Odds Specificpref Coverage & 37.2 & 55.8 & 56.8 & 48.5 & 55.0 & 44.2 & \textbf{59.8} & 59.2 & 59.5 \\
			Odds Specificpref Ranking & 10.2 & 49.7 & 50.7 & 19.6 & 27.2 & 11.0 & 50.8 & 51.6 & \textbf{51.7} \\
			\bottomrule
		\end{tabular}
	}
	\end{center}
	\label{tab:results}
\end{table}


==> old-tables.tex <==
\begin{table}
\caption{When using kendall Tau's for full ranking and RBO for top3 ranking}
\begin{tabular}{@{}llllllll@{}}
\toprule
    & Metrics                                             & linear & MLP1 & MLP2 & GBL Popularity & User Popularity &  \\ \midrule
1.  & \_testset\_coverage                                 & 60.9   & 68.2 & 70.3 & 84.5           & 77.9            &  \\
2.  & \_recommendations\_coverage                         & 67.9   & 73.2 & 74.2 & 80.0           & 74.6            &  \\
3.  & \_conditional\_prob\_generalpref\_intersectiontopk  & 62.2   & 60.8 & 57.2 & 29.0           & 41.8            &  \\
4.  & \_conditional\_prob\_generalpref\_rankingtop3       & 15.1   & 14.4 & 13.7 & 5.8            & 9.9             &  \\
5.  & \_conditional\_prob\_generalpref\_rankingfull       & 30.9   & 30.3 & 32.3 & 20.0           & 33.7            &  \\
6.  & \_conditional\_prob\_specificpref\_intersectiontopk & 50.0   & 49.0 & 48.4 & 28.9           & 41.5            &  \\
7.  & \_conditional\_prob\_specificpref\_rankingtop3      & 12.2   & 11.9 & 11.6 & 5.8            & 9.8             &  \\
8.  & \_conditional\_prob\_specificpref\_rankingfull      & 4.4    & 5.3  & 5.3  & 20.1           & 33.6            &  \\
9.  & \_odds\_ratio\_generalpref\_intersectiontopk        & 73.2   & 72.7 & 71.2 & 48.5           & 55.0            &  \\
10. & \_odds\_ratio\_generalpref\_rankingtop3             & 25.6   & 27.5 & 27.5 & 18.2           & 26.7            &  \\
11. & \_odds\_ratio\_generalpref\_rankingfull             & 28.0   & 28.4 & 30.5 & 17.5           & 34.3            &  \\
12. & \_odds\_ratio\_specificpref\_intersectiontopk       & 54.9   & 55.3 & 54.7 & 48.6           & 54.8            &  \\
13. & \_odds\_ratio\_specificpref\_rankingtop3            & 16.2   & 16.5 & 16.2 & 18.3           & 26.7            &  \\
14. & \_odds\_ratio\_specificpref\_rankingfull            & 5.6    & 6.4  & 6.3  & 17.7           & 34.4            &  \\ \bottomrule
\end{tabular}
\end{table}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\caption{When using RBO for both top3 ranking and full ranking}
\begin{tabular}{@{}llllllll@{}}
\toprule
    & Metrics                                             & linear & MLP1 & MLP2 & GBL Popularity & User Popularity &  \\ \midrule
1.  & \_testset\_coverage                                 & 60.9   & 68.2 & 70.3 & 84.5           & 77.9            &  \\
2.  & \_recommendations\_coverage                         & 67.9   & 73.2 & 74.2 & 80.0           & 74.6            &  \\
3.  & \_conditional\_prob\_generalpref\_intersectiontopk  & 62.2   & 60.8 & 57.2 & 29.0           & 41.8            &  \\
4.  & \_conditional\_prob\_generalpref\_rankingtop3       & 15.1   & 14.4 & 13.7 & 5.8            & 9.9             &  \\
5.  & \_conditional\_prob\_generalpref\_rankingfull       & 63.4   & 62.3 & 62.7 & 57.2           & 62.7            &  \\
6.  & \_conditional\_prob\_specificpref\_intersectiontopk & 50.0   & 49.0 & 48.4 & 28.9           & 41.5            &  \\
7.  & \_conditional\_prob\_specificpref\_rankingtop3      & 12.2   & 11.9 & 11.6 & 5.8            & 9.8             &  \\
8.  & \_conditional\_prob\_specificpref\_rankingfull      & 53.2   & 53.3 & 53.2 & 57.2           & 62.7            &  \\
9.  & \_odds\_ratio\_generalpref\_intersectiontopk        & 73.2   & 72.7 & 71.2 & 48.5           & 55.0            &  \\
10. & \_odds\_ratio\_generalpref\_rankingtop3             & 25.6   & 27.5 & 27.5 & 18.2           & 26.7            &  \\
11. & \_odds\_ratio\_generalpref\_rankingfull             & 64.4   & 64.2 & 64.6 & 58.2           & 64.4            &  \\
12. & \_odds\_ratio\_specificpref\_intersectiontopk       & 54.9   & 55.3 & 54.7 & 48.6           & 54.8            &  \\
13. & \_odds\_ratio\_specificpref\_rankingtop3            & 16.2   & 16.5 & 16.2 & 18.3           & 26.7            &  \\
14. & \_odds\_ratio\_specificpref\_rankingfull            & 54.9   & 55.1 & 55.1 & 58.3           & 64.5            &  \\ \bottomrule
\end{tabular}
\end{table}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\caption{When using RBO for both top3 ranking and full ranking -- revised with 70\% training data for the MFSGD}
\centering
\resizebox{1.26\columnwidth}{!}{%
\begin{tabular}{@{}llllllllllll@{}}
\toprule
    & Metrics                            & limers & ijcaiOP & ijcai & linear & MLP1 & MLP2 & GBL Popl. & User Popl. & Random &  \\ \midrule
1.  & \_testset\_coverage                & 8.4    & 48.4      & 52.4         & 60.7   & 70.8 & 71.2 & 84.5      & 77.9       & 32.4   &  \\
2.  & \_recommendations\_coverage        & 26.0   & 44.9      & 46.8         & 61.3   & 68.6 & 67.8 & 73.2      & 69.6       & 30.6   &  \\
3.  & CondPr\_generalpref\_intrsecttopk  & 50.3   & 55.5      & 53.9         & 62.9   & 58.1 & 56.6 & 29.0      & 41.8       & 43.9   &  \\
4.  & CondPr\_generalpref\_rank3         & 15.8   & 14.1      & 13.7         & 15.2   & 14.0 & 13.8 & 5.8       & 9.9        & 11.0   &  \\
5.  & CondPr\_generalpref\_rankFL        & 55.5   & 55.9      & 56.0         & 63.5   & 62.7 & 63.1 & 57.2      & 62.7       & 52.9   &  \\
6.  & CondPr\_specificpref\_intrsecttopk & 52.4   & 50.0      & 50.4         & 50.0   & 48.4 & 48.6 & 28.9      & 41.5       & 44.3   &  \\
7.  & CondPr\_specificpref\_rank3        & 15.1   & 13.4      & 13.3         & 12.2   & 11.8 & 11.8 & 5.8       & 9.8        & 11.3   &  \\
8.  & CondPr\_specificpref\_rankFL       & 55.4   & 53.2      & 53.2         & 53.2   & 53.2 & 53.3 & 57.2      & 62.7       & 52.8   &  \\
9.  & Odds\_generalpref\_intrsecttopk    & 32.6   & 62.7      & 62.0         & 73.4   & 72.3 & 70.4 & 48.5      & 55.0       & 43.7   &  \\
10. & Odds\_generalpref\_rank3           & 9.4    & 18.9      & 19.4         & 25.6   & 27.6 & 28.2 & 18.2      & 26.7       & 10.6   &  \\
11. & Odds\_generalpref\_rankFL          & 54.6   & 56.7      & 57.4         & 64.5   & 64.6 & 64.9 & 58.2      & 64.4       & 52.6   &  \\
12. & Odds\_specificpref\_intrsecttopk   & 36.9   & 53.4      & 54.3         & 54.9   & 54.8 & 55.5 & 48.6      & 54.8       & 44.4   &  \\
13. & Odds\_specificpref\_rank3          & 9.5    & 15.6      & 15.4         & 16.2   & 16.4 & 16.3 & 18.3      & 26.7       & 11.1   &  \\
14. & Odds\_specificpref\_rankFL         & 54.6   & 54.6      & 54.6         & 54.9   & 55.1 & 55.1 & 58.3      & 64.5       & 52.8   &  \\ \bottomrule
\end{tabular}
}
\end{table}


\begin{table}[h]    % This is the Ml-100K when combination is 2. 
	\caption{The test set coverage, top-k recommendations coverage, and the 8 explanation personalization metrics are reported here (averaged over all users). For \toolname, we computed metrics with three auxiliary models: Linear, a 2-layer neural network (MLP1), a 4-layer neural network (MLP2). For all columns, a higher value is better. The highest value for each metric is emboldened. }
	\begin{center}
	\resizebox{1.0\columnwidth}{!}{%
		\begin{tabular}{llllllllll}
			\toprule
			Metrics & LIME-RS & AMCF & AMCF-PH & GBL Popl. & User Popl. & Random & Our-Linear & Our-MLP1 & Our-MLP2 \\
			\midrule
			Testset Coverage & 8.4 & 47.2 & 52.6 & \textbf{84.5} & 77.9 & 32.4 & 60.3 & 66.6 & 71.4 \\
			Recommendations Coverage & 26.0 & 44.3 & 46.1 & \textbf{73.2} & 69.6 & 30.6 & 61.2 & 65.9 & 69.6 \\
			CondProb Generalpref Coverage & 50.3 & 58.2 & 47.2 & 29.0 & 41.8 & 43.9 & \textbf{63.1} & 56.5 & 55.7 \\
			CondProb Generalpref Ranking & \textbf{15.8} & 15.1 & 11.2 & 5.8 & 9.9 & 11.0 & 15.2 & 13.3 & 12.9 \\
			CondProb Specificpref Coverage & 52.5 & 53.1 & 52.4 & 29.0 & 41.7 & 44.1 & \textbf{55.3} & 53.5 & 53.0 \\
			CondProb Specificpref Ranking & 14.6 & 49.6 & 50.3 & 6.8 & 10.4 & 11.0 & \textbf{52.2} & 50.0 & 50.6 \\
			Odds Generalpref Coverage & 32.6 & 63.7 & 60.4 & 48.5 & 55.0 & 43.7 & \textbf{73.9} & 67.4 & 67.6 \\
			Odds Generalpref Ranking & 9.4 & 19.4 & 18.0 & 18.2 & \textbf{26.7} & 10.6 & 25.4 & 25.7 & \textbf{26.7} \\
			Odds Specificpref Coverage & 37.2 & 55.8 & 56.8 & 48.5 & 55.0 & 44.2 & \textbf{59.8} & 58.6 & 58.5 \\
			Odds Specificpref Ranking & 10.2 & 49.7 & \textbf{50.7} & 19.6 & 27.2 & 11.0 & \textbf{50.7} & 50.5 & \textbf{50.7} \\
			\bottomrule
		\end{tabular}
	}
	\end{center}
	\label{tab:results}
\end{table}

